Polarization-free Quantization of Linear Field Theories

It is well-known that there exist infinitely-many inequivalent representations of the canonical (anti)-commutation relations of Quantum Field Theory (QFT). A way out, suggested by Algebraic QFT, is to instead define the quantum theory as encompassing all possible (abstract) states. In the present paper, we describe a quantization scheme for general linear (aka. free) field theories that can be seen as intermediate between traditional Fock quantization and full Algebraic QFT, in the sense that: * it provides a constructive, explicit description of the resulting space of quantum states; * it does not require the choice of a polarization, aka. the splitting of classical solutions into positive vs. negative-frequency modes: in fact, any Fock representation corresponding to a "reasonable" choice of polarization is naturally embedded; * it supports the implementation of a "large enough" class of linear symplectomorphisms of the classical, infinite-dimensional phase space. The proposed quantization (like Algebraic QFT) is notably meant for use on curved spacetimes, where the lack of a preferred choice of polarization makes the introduction of a Fock representation problematic. Accordingly, we illustrate it in the simple case of a free Klein-Gordon field on a spatially-compact, cosmological spacetime.

==> meta1.tex <==
\newcommand{\AuthorsAffil}{\begin{center}\vspace{-0.1cm}%
\Mpar \vspace{\Ssaut}\ensstitre{Suzanne Lanéry}\vspace{0.1cm}%
\Mpar \vspace{\Ssaut}\enmoinsgrand{Centro de Ciencias Matemáticas, Universidad Nacional Autónoma de México, Morelia, México}\vspace{0.2cm}%
\Mpar \vspace{\Ssaut}\makeatletter\@date\makeatother\vspace{-0.4cm}\end{center}}


==> meta2.tex <==
\def\Acknowledge{\vspace{-0.7cm}\MsectionBNoNumberNoToc{acknowledgements}{Acknowledgements}\vspace{\PsectionB}%
\Mpar \vspace{\Saut}\hspace{\Alinea}I would like to thank Robert Oeckl, for providing the initial motivation for the present study as well as for insightful discussions.%
\Mpar \vspace{\Saut}\hspace{\Alinea}Financial support through the Programa de Becas Posdoctorales de la UNAM is acknowledged.}


==> not01.tex <==
\RequirePackage{graphicx}
\RequirePackage{dsfont}
\RequirePackage{nicefrac}
\newcommand\hmmax{2}
\newcommand\bmmax{2}
\RequirePackage{bm}
\newcommand{\definitionFonction}[6][1.2]{\renewcommand{\arraystretch}{#1}\begin{array}{ccrcl} #2 &\hspace{0.25cm}:\hspace{0.25cm}& #3 &\hspace{0.25cm}\rightarrow\hspace{0.25cm}& #4 \\ && #5 &\hspace{0.25cm}\mapsto\hspace{0.25cm}& #6 \end{array}\renewcommand{\arraystretch}{1}\hspace{0.15cm}}\newcommand{\definitionFonctionCrtsPrd}[8][1.2]{\renewcommand{\arraystretch}{#1}\begin{array}{ccrclcl} #2 &\hspace{0.25cm}:\hspace{0.25cm}& #3 &\hspace{0.1cm}\times\hspace{0.1cm}& #4 &\hspace{0.25cm}\rightarrow\hspace{0.25cm}& #5 \\ && #6, && #7 &\hspace{0.25cm}\mapsto\hspace{0.25cm}& #8 \end{array}\renewcommand{\arraystretch}{1}\hspace{0.15cm}}\newcommand\withAS[3]{\renewcommand{\arraystretch}{#1}\begin{array}{#2}#3\end{array}\renewcommand{\arraystretch}{1}}
\newcommand{\matrixTwo}[4]{\left(\begin{array}{c@{\hspace{0.25cm}}c}#1&#2\\#3&#4\end{array}\right)}
\newcommand{\matrixThree}[9]{\left(\begin{array}{c@{\hspace{0.25cm}}c@{\hspace{0.25cm}}c}#1&#2&#3\\#4&#5&#6\\#7&#8&#9\end{array}\right)}
\newcommand{\matrixDiag}[3]{\left(\begin{array}{c*{3}{@{\hspace{0.25cm}}c}}#1&&&\\&#2&&\\&&\ddots&\\&&&#3\end{array}\right)}
\newcommand{\alternative}[5][1.2]{\renewcommand{\arraystretch}{#1}\left\{\begin{array}{l@{\hspace{0.25cm}}l}#2&#3\\#4&#5\end{array}\right.\mathchoice{\hspace{0.15cm}}{}{}{}\renewcommand{\arraystretch}{1}}
\newcommand{\ssquare}{\scalebox{0.4}{$\square$}}
\def\middlewithspace#1{\;\middle#1\;}
\newcommand{\mkop}[1]{\mathop{\text{{#1}}}\nolimits}
\newcommand{\grpAct}[1]{#1\mathchoice{{\scriptstyle\rangle}}{{\scriptstyle\rangle}}{{\scriptscriptstyle\rangle}}{{\scriptscriptstyle\rangle}}}
\newcommand{\setquot}[2]{\mathchoice{\left.\raisebox{.2em}{$\displaystyle#1$}\middle/\raisebox{-.2em}{$\displaystyle#2$}\right.\hspace{0.15cm}}{\left.#1\middle/#2\right.}{\left.#1\middle/#2\right.}{\left.#1\middle/#2\right.}}\newcommand{\hmtpCls}[1]{\left[#1\right]_{{\text{{homtp}}}}}
\newcommand{\smallfrac}[2]{{\textstyle\frac{#1}{#2}}}
\newcommand{\smallsum}{\mathop{\textstyle\sum}\nolimits}
\DeclareBoldMathCommand[bold]\boldplus{+}\DeclareBoldMathCommand[bold]\boldminus{-}\DeclareBoldMathCommand[bold]\boldtheta{\theta}\newcommand{\heavyplus}{\pmb{\boldplus}}\newcommand{\heavyminus}{\pmb{\boldminus}}\RequirePackage{tikz}\newlength{\LongueurAuxA}\newlength{\LongueurAuxB}\newlength{\LongueurAuxC}\newlength{\LongueurAuxD}\newcommand{\deuxlignes}[3]{\settowidth{\LongueurAuxA}{$\scriptstyle#2$}\settowidth{\LongueurAuxB}{$\scriptstyle#3$}\pgfmathsetlength{\LongueurAuxC}{max(\LongueurAuxA,\LongueurAuxB)}\parbox{\LongueurAuxC}{\makebox[\LongueurAuxC][c]{$\scriptstyle#2$}\\[#1]\makebox[\LongueurAuxC][c]{$\scriptstyle#3$}}}\newcommand{\troislignes}[4]{\settowidth{\LongueurAuxA}{$\scriptstyle#2$}\settowidth{\LongueurAuxB}{$\scriptstyle#3$}\settowidth{\LongueurAuxC}{$\scriptstyle#4$}\pgfmathsetlength{\LongueurAuxD}{max(max(\LongueurAuxA,\LongueurAuxB),\LongueurAuxC)}\parbox{\LongueurAuxD}{\makebox[\LongueurAuxD][c]{$\scriptstyle#2$}\\[#1]\makebox[\LongueurAuxD][c]{$\scriptstyle#3$}\\[#1]\makebox[\LongueurAuxD][c]{$\scriptstyle#4$}}}


==> not02.tex <==
\newcommand{\dof}{dof.\xspace}\newcommand{\dofs}{dofs\xspace}

